Super Interaction Neural Network

Recent studies have demonstrated that the convolutional networks heavily rely on the quality and quantity of generated features. However, in lightweight networks, there are limited available feature information because these networks tend to be shallower and thinner due to the efficiency consideration. For farther improving the performance and accuracy of lightweight networks, we develop Super Interaction Neural Networks (SINet) model from a novel point of view: enhancing the information interaction in neural networks. In order to achieve information interaction along the width of the deep network, we propose Exchange Shortcut Connection, which can integrate the information from different convolution groups without any extra computation cost. And then, in order to achieve information interaction along the depth of the network, we proposed Dense Funnel Layer and Attention based Hierarchical Joint Decision, which are able to make full use of middle layer features. Our experiments show that the superior performance of SINet over other state-of-the-art lightweight models in ImageNet dataset. Furthermore, we also exhibit the effectiveness and universality of our proposed components by ablation studies.

==> SINet_Architecture.tex <==
\section{SINet Architecture}
In this section, we introduce  the SINet Architecture which consists of the three components mentioned in preceding section. We firstly build up the SI Unit and we use this Unit to construct the whole networks.

\label{architecture}
\subsection{SI Unit}
%综合前面提出的exchange以及narrow操作的优势，我们专门为轻量化网络设计了一种SINet Unit。
%这种Unit可以无缝的嵌入到任何cnn网络构架中，做到在不减少网络精度的前提下大幅降低网络计算量。
%%%%%%%%%%%%%%%%%%%%%
%Unit内部不同组的信息交互关系如图2所示，其中绿色模块是unit内部的特征计算层，红色线条表示了我们独特的shortcut形式，展现了在没有引入任何额外计算量的情况下我们式如何实现了组间的信息交互。
%Unit内部结构的深度方向信息交互设计如图3所示，其中红色H表示特征计算（conv+relu+bn），浅紫红色模块表示经过每一层特征计算层的输出特征处理模块，不同颜色特征表示不同层产生的特征,不同颜色的线条表示相应特征的信息流，可以看出随着层级的加深，后面每一层都会包含前面所有层的信息。
%蓝色部分表示的是narrow操作（具体实现见图2中蓝色模块），这个操作紧连在每个层级的连接计算之后，为了可以在有限的计算资源下实现全联通的信息交互形式（图3显示了我们是如何实现每个unit单个组内部式如何实现全联通的）。
%unit的整体结构如图5所示，我们结合使用了图2的组间信息交互以及图3的深度方向上层级之间的信息交。这种unit结构是一种具有dense funnel连接的倒置组间交互残差的瓶颈深度可分离卷积。
%%%%%%%%%%%%%%%%%%%%%

Taking advantage of the \textbf{Exchange Shortcut Connection} and \textbf{Dense Funnel Layer} operation, we propose a novel \textit{SINet Unit} specially designed for lightweight networks. This \textit{Unit} can be seamlessly embedded into any existing CNN network architecture. The amount of network computing can be greatly reduced without network accuracy decline.

In SI Unit, the information interaction along depth direction is shown in Figure \ref{fig:narrow}. 
The light amaranth module presents the feature obtained from each block processing module through,
where the different color features represent the different blocks, and the lines of different colors represent the information flow of different features. 
It can be seen that as the level deepens, each subsequent layer will contain information about all the previous layers.
The blue part indicates the narrow operation which is closely connected to the connection calculation of each level, in order to realize the information exchange form of the full communication under the limited computing resources. 

And the information interaction relationship between different groups is shown in Figure \ref{fig:group and exchange}. 
The green module (block) is the feature calculation layer, and the red line indicates our unique shortcut form which show how we can achieve information interaction between groups without any additional calculations. 
And the detail achievement of narrow operation is shown in blue module.

The overall structure of \textit{SINet Unit}  is shown in the Fig \ref{fig:exchange units}. 
We use the information interaction between different groups of Figure \ref{fig:group and exchange} in combination with the information exchange between the levels along depth direction of Figure \ref{fig:narrow}. 
To sum up, this unit structure is a bottleneck depth separable convolution with an inter-group interaction residual of a dense funnel connection, and realize fully information interaction of the internal block and internal unit (outer block).

\begin{figure}[h]
    \centering
    \includegraphics[width=.5\textwidth]{image/exchange.pdf}
    \caption{The information exchange in the whole SI Unit, where $X_0$ is the input feature maps and $X_l$ is the output feature maps in this Unit, S implies split operation to divide the feature maps into 2 groups, and M implies merge operation to connect the feature maps from different groups.}
    \label{fig:exchange units}
\end{figure}

In summary, the design points are as follows:
\begin{itemize}
\item Composite Function \textit{H}. 
Motivated by \cite{Sandler2018MobileNetV2}, we define $H_l(·)$ as a composite function of three consecutive operations:batch normalization (BN) \cite{Ioffe2015Batch}, followed by a rectified linear unit (ReLU) \cite{Krizhevsky2012alexnet} and a $3 \times 3$ convolution (Conv).For the  $3 \times 3$ layer, we use a computational economical  $3 \times 3$ depthwise convolution \cite{Chollet2016Xception,howard2017mobilenets} on the residual bottleneck layers.

\item Exchange shortcut. 
In order to ensure the sufficiency of feature exchange of different groups, unlike traditional skip dense connection, we concat the output feature maps of this branch with the input feature maps of other branch, shown in Equ \ref{equ:exchange_resnet} instead concat the output and input feature maps in one branch.
Importantly, in order to balance the characteristics of different branches for the fairness of the final prediction, we ensure the output channels equal to input.

\item Dense Funnel. 
Start from the branch exchange function and dense connect operation, the final channels of output feature maps in this unit will double up.
For reducing the memory and calculation, we will set a narrow layers to reduce the output channels.
we define the dense funnel layers as a $1 \times 1$ convolution, the output channels can be changed by our need.
\end{itemize}

Thanks to the above operation, all components in SI unit can be computed efficiently.
This Unit can be applied in different models, like ResNet \cite{Huang2016ResNet}, MobileNet \cite{howard2017mobilenets}, ShuffleNet \cite{Zhang2017ShuffleNet} and so on, to reduce the complexity of computation.
Compared with original networks, our structure has less complexity under the same settings,
given a covloutional computation with the kernel size $k \times k$, when the input size $c \times h \times w$ and the output channels m, this unit requires $c \times h \times w \times k \times k \times m$ FLOPs, while Exchange Units with same setting requires $c \times h \times w \times k \times k \times m / 2$ FLOPs, and good performance which can be shown in \ref{experiment}.
\label{si unit}


\subsection{Network Architecture}
%基于SI unit和基于注意的分层联合决策中，我们在表中呈现整体SINet整体结构。
%Si unit采用的是分组计算，其基本构建块是具有反向残差的瓶颈深度可分离卷，我们的残差结构是一种新型的具有组间的信息交互的exchange shortcut连接；其基本构建快的连接形式我们采用的是一种新颖密集的漏斗层。
%我们提出的网络主要由分成四个阶段的一组SI单元组成。每个阶段的第一个构建块使用stride=2，与mobilenet2类似，我们使用扩展因子6应用于每个单元的输入张量大小。
Built on SI Unit in Section \ref{si unit} and Hierarchical Joint Decision based on Attention as discussed in Section \ref{approach}, we present the overall SINet architecture in Table \ref{tab:overall architecture}. 

The basic building block in SI Unit is a bottleneck depth-separable convolution with inverse residuals(describe in Tab \ref{tabel:Bottleneck residual block}) with exchange and a dense funnel layer.
The proposed network is mainly composed of a stack of SI units grouped into four stages. 
The first building block in each stage is applied with stride = 2. 
Different from \cite{Sandler2018MobileNetV2}, the expansion factor of 5 applied to the size of the input tensor for each units.
The architecture of SINet contains the initial fully convolution layer with 24 filters, followed by 4 Exchange Units (\yang{not sure}16 residual bottleneck which is described in the Table \ref{tabel:Bottleneck residual block} layers totally), shown in Fig \ref{tab:overall architecture}.
We use ReLU6 as the non-linearity because of its robustness when used with low-precision computation \cite{}. \yang{add cite}
We always use kernel size $3 \times 3$ as is standard for modern networks, and utilize dropout and batch normalization during training.

% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[h]
  \centering
  \caption{Bottleneck residual block transforming from k
to k' channels, with stride s, and expansion factor t.}
    \begin{tabular}{rrr}
            &         &  \\
    \midrule
    \multicolumn{1}{c|}{Input } & \multicolumn{1}{c|}{Operator } & \multicolumn{1}{c}{Output} \\
    \midrule
    \multicolumn{1}{c|}{h \times w \times k } & \multicolumn{1}{c|}{1 \times 1 conv2d , ReLU6 } & \multicolumn{1}{c}{h \times w \times (tk)} \\
    \multicolumn{1}{c|}{\textit{h \times w \times tk }} & \multicolumn{1}{c|}{3 \times 3 dwise s=s, ReLU6 } & \multicolumn{1}{c}{\dfrac{h}{s} \times \dfrac{w}{s} × (tk)} \\
    \multicolumn{1}{c|}{\dfrac{h}{s} \times w/s \times (tk)} & \multicolumn{1}{c|}{linear 1 \times 1 conv2d } & \multicolumn{1}{c}{\dfrac{h}{s} \times \frac{w}{s} \times k'} \\
    \midrule
            &         &  \\
    \end{tabular}%
  \label{tabel:Bottleneck residual block}
\end{table}%

In SI units, group number we set is 2, it controls the groups that all convolution calculation divided into.
Our intent is to provide a reference design as simple as possible, although we find that further hyper-parameter tunning might generate better results.

 % Table generated , SINet architecture & /tabincell
\begin{table}[h]
\footnotesize
  \centering
  \caption{SINet architecture}
    \begin{tabular}{rcrrrr}
            &         &         &         &         &  \\
    \midrule
    \multicolumn{1}{c|}{Layer } & \multicolumn{1}{c|}{output size} & \multicolumn{1}{c|}{k} & \multicolumn{1}{c|}{s} & \multicolumn{1}{c|}{repeat} & \multicolumn{1}{c}{out channel} \\
    \midrule
    \midrule
    \multicolumn{1}{c|}{image} & \multicolumn{1}{c|}{224 x 224 x 3} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{3} \\
    \multicolumn{1}{c|}{Conv} & \multicolumn{1}{c|}{112 x 112 x 24} & \multicolumn{1}{c|}{3 x 3} & \multicolumn{1}{c|}{2} & \multicolumn{1}{c|}{1} & \multicolumn{1}{c}{24} \\
    \midrule
    \multicolumn{1}{c|}{\multirow{2}[0]{*}{SI 1}} & \multicolumn{1}{c|}{56 x 56 x 32} & \multicolumn{1}{c|}{3 x 3} & \multicolumn{1}{c|}{2} & \multicolumn{1}{c|}{1} & \multicolumn{1}{c}{32} \\
    \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{56 x 56 x 32} & \multicolumn{1}{c|}{3 x 3} & \multicolumn{1}{c|}{1} & \multicolumn{1}{c|}{2} & \multicolumn{1}{c}{32} \\
    \midrule
    \multicolumn{1}{c|}{\multirow{2}[0]{*}{SI 2}} & \multicolumn{1}{c|}{28 x 28 x 64} & \multicolumn{1}{c|}{3 x 3} & \multicolumn{1}{c|}{2} & \multicolumn{1}{c|}{1} & \multicolumn{1}{c}{64} \\
    \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{28 x 28 x 64} & \multicolumn{1}{c|}{3 x 3} & \multicolumn{1}{c|}{1} & \multicolumn{1}{c|}{2} & \multicolumn{1}{c}{64} \\
    \midrule
    \multicolumn{1}{c|}{\multirow{2}[0]{*}{SI 3}} & \multicolumn{1}{c|}{14 x 14 x 96} & \multicolumn{1}{c|}{3 x 3} & \multicolumn{1}{c|}{2} & \multicolumn{1}{c|}{1} & \multicolumn{1}{c}{96} \\
    \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{14 x 14 x 96} & \multicolumn{1}{c|}{3 x 3} & \multicolumn{1}{c|}{1} & \multicolumn{1}{c|}{2} & \multicolumn{1}{c}{96} \\
    \midrule
    \multicolumn{1}{c|}{\multirow{2}[0]{*}{SI 4}} & \multicolumn{1}{c|}{7 x 7 x 320} & \multicolumn{1}{c|}{3 x 3} & \multicolumn{1}{c|}{2} & \multicolumn{1}{c|}{1} & \multicolumn{1}{c}{320} \\
    \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{7 x 7 x 320} & \multicolumn{1}{c|}{3 x 3} & \multicolumn{1}{c|}{1} & \multicolumn{1}{c|}{2} & \multicolumn{1}{c}{320} \\
    \midrule
    \multicolumn{1}{c|}{Conv} & \multicolumn{1}{c|}{7 x 7 x 1280} & \multicolumn{1}{c|}{1 x 1} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{1} & \multicolumn{1}{c}{1280} \\
    \multicolumn{1}{c|}{Avgpool} & \multicolumn{1}{c|}{1 x 1 x 1280} & \multicolumn{1}{c|}{7 x 7} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{1} & \multicolumn{1}{c}{-} \\
    \multicolumn{1}{c|}{Conv} & \multicolumn{1}{c|}{1 x 1 x c} & \multicolumn{1}{c|}{1 x 1} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{c} \\
    \midrule
            &         &         &         &         &  \\
    \end{tabular}%
  \label{tab:overall architecture}%
\end{table}


% \subsection{Trade-off hyper parameters}
% we tailor our architecture to different performance points, by using the input image resolution and width multiplier as tunable hyper parameters, that can be adjusted depending on desired accuracy/performance trade-offs.

% As in \cite{} we tailor our architecture to different performance points, by using the input image resolution and width multiplier as tunable hyper parameters, that can be adjusted depending on desired accuracy/performance trade-offs. 
% Our primary network (width multiplier 1, 224 × 224), has a computational cost of 220\yang{need to change} million multiply-adds and uses 2.8 \yang{need to change} million parameters.
% And we apply width multiplier to all layers except the very last convolutional layer.
% This improves performance for smaller models.
% We explore the performance trade offs, for input resolutions from 96 to 224,and width multipliers of 0.35 to 1.4. 
% The network computational cost ranges from 7 multiply adds to 585M MAdds, while the model size vary between 1.7M and 6.9M parameters.


==> appraoch.tex <==
\section{Preliminaries, discussion and intuition}
\label{approach}
%小型网络的设计主要遵循着低计算量高性能的原则。所以一般的小型网络都有着相对较浅的结构（比如：）。
%为了获得一个高性能的小型网络，我们从如何更加有效的利用已有特征信息这一全新角度通过特征重用以及特征信息交互增大网络的信息流通性，从而挖掘网络的潜力。
Currently, lightweight networks designing mainly follows the principle of low computational cost and high accuracy. Therefore, it means that these networks tend to be shallow in depth for computation saving, such as MobileNet (XX layers) and ShuffleNet (XX layers) \xu{need to fill in}.

Based on this trend, in order to obtain higher accuracy in such small network architecture, we should make full use of the existing feature information and enhance the information interaction through the network in all directions. This is the most important  motivation and guidance of our SINet.

\subsection{Exchange Shortcut Connection}
%现在的卷积神经网络通常由具有相同结构的重复构建块组成。其中，state-of-the-art的网络比如resnet，resneXt，mobilenet，shufflenet等使用depthwise separable卷积块堆叠而成，mobilenetv2使用了depthwise separable with inverted residual structure作为重复构建快等等，他们都是将有效的群组卷积或深度可分离卷积（也可以看作组卷积）引入构建块，以在表示能力和计算成本之间取得良好的折衷。
%组卷积是最为简单使用的通道稀疏连接方式，所以被广泛利用，如公式所示，可以看出他可以将一个卷积层计算量降至原来的。。。倍。。
%但是，组卷积堆栈具有明显的副作用：来自某个组的输出仅来自一小部分输入通道，这个属性阻止不同组之间的信息流并削弱表示特征。（见图）
%shufflenet提出channel shuffle的思想，igcv2提出交错组卷积的思想，他们的目的都是为了打乱使用在point convolution上组卷积造成的信息不流通。
%不同于这种专门设计用在单一卷积层上的组卷积操作，我们直接从输入特征图开始进行分组的计算，如图（）所示。
%也不同于他们使用打乱信息——shuffle and permutation的方式来解决组间信息不流通的问题，我们提出一种新形的基于short connect的组间信息交互策略——Interaction。
%short connect最早在resnet和高速公路网络中被提出用来降低随着网络深度的增加造成的梯度消失现象，其公式表示如下：
%在我们的设计中，我们使用的short connect的另外一个主要功能：提高信息的交互。
%首先是利用short connect来进行组间的信息交互，从图以及公式中可以明显的看出不同分支的计算操作互不干涉，某一分支的输出仅与该分支内的输入有关。我们提出的这种新型的基于分组计算的shortconnect操作的形式如图所示，不同于以往的旁支直连操作（。。），我们的计算操作如公式所示。（其中黑体表示不同）。

There have been many works focused on the lightweight CNNs models design, including Xception \cite{Chollet2016Xception}, MobileNet \cite{howard2017mobilenets}, MobileNetV2 \cite{Sandler2018MobileNetV2} and ShuffleNet \cite{Zhang2017ShuffleNet}, etc.  Almost all of these models utilize the \textit{Group Convolution} operation for reducing the computational costs.

As well known, the computation of CNN is mainly concentrated in the convolution  process \cite{} \xu{need to cite}.
\yang{need to change}
Group convolution can reduce the computation cost by convolving only on a part of, instead of all feature maps outputted by the preceding layer. 
However, while reducing the amount of computation, group convolution also weakens the feature extraction ability of the network because  it only uses a small portion of feature maps for every convolution kernel. 
Fig.\ref{fig:group} illustrates two stacked group convolutions.
It is clear that outputs from a certain group are only related to its own inputs.
The information interaction between groups is completely interrupted.

\begin{figure}[h!]
 \centering
    \includegraphics[height=.4\textwidth]{image/Block1.pdf}
    \caption{Group convolution schematic diagram, the  blue and yellow nodes represent the different groups respectively}
\label{fig:group}
\end{figure}

To deal with this intractable problem, MobileNetV1 and MobileNetV2 leverage the point-wise convolution to reintegration the separated channels.
Since point-wise convolutions occupy 93.4\% computation \cite{howard2017mobilenets}, \cite{Zhang2017ShuffleNet,Zhang2017IGCV} uses group convolution in $1 \times 1$convolution. ShuffleNet \cite{Zhang2017ShuffleNet} introduced channel shuffle operation to mix up the information among groups, IGCV2 \cite{Zhang2017IGCV} proposed Interleaved Group Convolutions, breaking the barrier between groups.

Different from above operations, in SINet, we propose a totally novel and more efficient method, named Exchange Shortcut Connection, which can achieve the information interaction without extra computation, as illustrated in Fig. \ref{fig:exchange units}.

Inspired by \cite{Huang2016ResNet}, we mix up the information from different groups by using the shortcut connection naturally. We define $\mathbf{H}(\cdot)$ as a composite function of three consecutive operations: a $3 \times 3$ convolution (Conv), followed by a rectified linear unit (ReLU) and batch normalization (BN).
Let $\mathbf{H}_l(\cdot), l \in {1, ..., N}$ denote the function computed by the $l_{th}$  layer.
$\boldsymbol{X_{0}}$ represents input image and $\boldsymbol{X_{l}}$ is output of the $l_{th}$ layer. Standard ResNet \cite{}\xu{need to cite Kaiming He paper} which owns shortcut connection can be recursively defined as Eq. \ref{resnet}

\begin{equation}
\label{resnet}
	\boldsymbol{X_{l}} = \mathbf{H}\left ( \boldsymbol{X_{l-1}} \right )+\boldsymbol{X_{l-1}}
\end{equation}

If we divide all operations in this network into two groups, and conduct convolution respectively,  these grouped network can be recursively defined as Eq. \ref{divide_resnet}

\begin{equation}
\label{divide_resnet}
\begin{aligned}
   &\boldsymbol{X}^1_{l-1},\boldsymbol{X}^2_{l-1}=\mathbf{Split}(\boldsymbol{X}_l)\\
   &\boldsymbol{ X}^1_{l} =  \mathbf{H^1_{l}}(\boldsymbol{X}^1_{l-1})+\boldsymbol{X}^1_{l-1}\\
    &\boldsymbol{ X}^2_{l} =  \mathbf{H^2_{l}}(\boldsymbol{X}^2_{l-1})+\boldsymbol{X}^2_{l-1}\\
   &\boldsymbol{ X}_{l} =[\boldsymbol{ X}^1_{l},\boldsymbol{ X}^2_{l}]
\end{aligned}
\end{equation}


For achieving the information interaction, we introduce exchange operation, which can be recursively defined as Eq. \ref{exchange_resnet}.

\begin{equation}
\label{exchange_resnet}
\begin{aligned}
   &\boldsymbol{X}^1_{l-1},\boldsymbol{X}^2_{l-1}=\mathbf{Split}(\boldsymbol{X}_l)\\
   &\boldsymbol{ X}^1_{l} =  \mathbf{H^1_{l}}(\boldsymbol{X}^1_{l-1})+\boldsymbol{X}^2_{l-1}\\
    &\boldsymbol{ X}^2_{l} =  \mathbf{H^2_{l}}(\boldsymbol{X}^2_{l-1})+\boldsymbol{X}^1_{l-1}\\
   &\boldsymbol{ X}_{l} =[\boldsymbol{ X}^1_{l},\boldsymbol{ X}^2_{l}]
\end{aligned}
\end{equation}

Fig.\ref{fig:group and exchange} illustrates  two stacked group convolutions with information exchange operation. Compared with Fig. \ref{fig:group},
Exchange shortcut allows different convolution groups to access input data from others, which builds up information interaction among the width of network. It is also worthy noting that this method need not any extra computation cost and can be easily and flexibly extended to any layers in neural networks.



% At the beginning of each unit, the input of c feature channels split into two branches with $c1$ and $c2$ (in equ \ref{equ:c}) channels respectively. 
% \begin{equation}
%     c1=c*0.5 \quad c2=c-c1
% \label{equ:c}
% \end{equation}

\begin{figure}
 \centering
    \includegraphics[width=.5\textwidth]{image/Block2.pdf}
    \caption{The detail of Exchange Shortcut Connection, the red  bold lines denote the Exchange Shortcut Connections\xu{words in fig need to be amplified, and the red lines need to be bold}}
\label{fig:group and exchange}
\end{figure}




\subsection{Dense Funnel Layer}
%resnet中旁支直连的操作是为了可以利用到上一层的信息，那么为了可以进一步的利用信息，我们希望不仅仅可以使用到上一层的信息，我们希望可以利用到同一层级中前面所有层的信息.但是直接的connect操作，类似于densent中的dense connect会导致内存使用以及计算量的爆炸，densnet验证了denseconnect的有效性，但是很明显，这种操作无法实现轻量化的网络。
%因此，我们引入了一种称为窄型全连接结构的新型连接结构。图说明了这种结构。
%我们通过concat操作来组合当前层先前卷积块的所有特征（不同颜色的特征块，表示不同block产生的特征）。因此，l层有l-1个输入，图中的不同颜色的连接线表示不同特征的数据流。
%首先是第一层信息的产生，绿色表示本组第一层计算所得的特征图，红色特征是经过卷积计算操作（H）后得到的特征，紫色特征块同理。使用shortcut连接方式，将本block内部前面所有一层信息于本层信息进行connect连接，为了避免 connect带来的内存计算量爆炸现象，使用narrow操作对concat后的特征进行挤压，之后，narrow操作之后就是本层卷积的结束，将得出的特征图作为下一层卷积的输入进行计算，重复之前操作%

Exchange shortcut connection only leverages the information of the nearest layer. To further improve the information interaction along the depth of network, we expect to connect the current layer with all preceding layers, like done in DenseNet \cite{Huang2016Densely}. 
% It can be formally represented as Eq. \ref{equ:dense}, where $[X_0,X_1,\cdots,X_{l-1}]$ refers to the concatenation of the feature maps produced in layers $0,1,\cdots,l-1$.

% \begin{equation}
% \begin{aligned}
%   \boldsymbol{X}_l=\mathbf{H}_l([\boldsymbol{X}_0,\boldsymbol{X}_1,\cdots,\boldsymbol{X}_{l-1}])
% \label{equ:dense}
% \end{aligned}
% \end{equation}

Although this kind of dense connection has been proved to be very effective in general CNNs model. Nevertheless, it is obvious that this operation can cause memory and computational explosion which is not acceptable for a lightweight network.
Thus, we introduced a novel connection structure called Dense Funnel Layer. 
Fig. \ref{fig:narrow} illustrates the layout schematically. The different colored lines in the figure represent the data flow of different layers.
The green indicates the feature maps calculated by the first layer of this block, the red is the feature maps obtained after the composition operation $\mathbf{H}$ (Conv+ReLU+BN) on green feature maps.
Firstly, we combine features from preceding convolutional layers (green feature maps $A$) and current layer output  features (red feature maps $B$) by concatenating them.  
Then we use $1\times 1$ convolution layer to reduce the channels and mix the information from both sources, to get the output feature maps $C$.\xu{need add ABC in the figure}
This operation  is the key for avoiding the memory explosion caused by the dense connection through squeezing out the useless information of the preceding feature maps.
After that, we feed these mixed feature maps to the next layer and conduct the the similar operations repeatedly (connect green, red and purple feature maps, apply $\mathbf{H}$ and Dense Funnel layer on it). 
After several iterations in the network, we can hold view that the last set of feature maps contains the information of all preceding feature maps approximately.

\begin{figure*}[h!]
    \centering
    \includegraphics[height=.2\textwidth]{image/narrow.pdf}
    \caption{A 3-layer block with Dense Funnel Layer. Each layer takes narrowed preceding feature maps as its own input.}
    \label{fig:narrow}
\end{figure*}

% In SINet, we propose a down sampling operation---$Narrow(\cdot)$ to solve this problem. We concatenate the previous layers output $\boldsymbol{X}_{l-1}$ with the current layer output $\boldsymbol{X}_l$,  like Eq. \label{resnet}, then following by a $1\times1$ convolution narrow layer for reducing the number of  channels. The output of narrow layer is denoted as $\boldsymbol{Y}_l$.  After recursion illustrated in Eq. \ref{equ: detail connection}, we hold view that the final output $\boldsymbol{Y}_L$ contains information about all previous layers approximately. 
% \begin{equation}
% \begin{aligned}
% X_1= & H_1(X_0) \quad Y_1=[X_1,X_0] \\
% Y_1= & Narrow(Y_1)  \\
% X_2= & H_2(Y_1) \\
% Y_2= & [X_2,Y_1]  =[X_2,\bm{X_1'},\bm{X_0'}] \\
% Y_2= & Narrow(Y_2) \\
% & \vdots  \\
% Y_{L-1}& =  Narrow(Y_{L-1}) \\
% X_L = &  H_L(Y_{L-1}) \\
% Y_{L} = &[X_{L},Y_{L-1}]=[X_{L},\bm{X_{L-1}'},\cdots,\bm{X_1'}] \quad (*)
% \end{aligned}
% \label{equ: detail connection}
% \end{equation}



% \begin{equation}
% \begin{aligned}
% & X^1_{l-1},X^2_{l-1}=Splite(X_l)\\
% X^1_{l}= & H^1_{l}(X^1_{l-1}) \quad X^1_{l}=[X^1_{l},X^1_{l-1}]\\
% X^2_{l}= & H^2_{l}(X^2_{l-1})  \quad  
% X^2_{l}=[X^2_{l},X^2_{l-1}] \\
% X_{l}& =[X^1_{l},X^2_{l}] \quad X_{l}=Narrow(X_{l})
% \end{aligned}
% \label{equ:exchaneg units}
% \end{equation}
% where $[X^1_{l},X^1_{l-1}]$ and $[X^2_{l},X^2_{l-1}]$ refers to the concatenation of the feature-maps produced by different two branch in layer l.

\subsection{Hierarchical Joint Decision based on Attention}
%经典的cnn网络可以分为三个部分：
%一系列级联的conv+pooling层。在级联的过程中，输入尺寸会逐渐变小，同时输出的channel数逐渐变大，完成信息从低级到高级的抽象。 一系列级联的全连接层。在卷积层到全连接层的交界处，卷积层输出会被转化成一维的输入送进全连接层。
% 最后的输出层，根据任务的需要，决定输出的形式。
%图1展示了传统的卷积神经网络在做分类任务的基本框架，可以看出经典cnn的全连接层使用的特征只是最后一层卷积层得到的特征，这是最高级的一种特征。
%对于卷积神经网络而言，用于决策的可利用特征应该要越全面越好，虽说高级特征可以较高程度的表征图片信息，但是这并不表示低级信息是没有用的，相反，这些低级信息应该被利用起来。
%也就是说将低级特征和高级特征进行有效的联合决策会提高深度网络的决策效果。
%一种最为直观的联合决策的方式就是不同层级的特征直接连接，这种简单的操作只能用在每一层特征图的大小不变时。然而，卷积网络的一个重要部分是下采样层，这些层改变了特征映射的大小。
% 为了将不同大小的特征图进行连接，一种简单的思想就是对于这些特征图进行不同程度的下采样，然后将下采样到统一尺度的特征度进行连接，最后用于决策。
%但是这种方法有一个缺点：首先，下采样得到的特征图已经失去了这一层级特征图特有的特征信息，再者，直接的下采样都会有一定程度的信息丢失，用失去了有效特征信息并且还有部分信息丢失的特征来结合最后的卷积特征进行决策，这会在一定程度上干扰网络的决策(添加引用实验表）。
%为了让各个层级的特征信息无损失的进行联合，我们将不同层级（Block）输出的特征图分别转化为一维的输出，然后将全部的一维特征直接连接起来输入全连接层。
%不同层级的特征信息的贡献对于网络最后的决策是不一样的，为了体现不同层级特征的贡献度，我们通过学习到不同层级特征的依赖关系来平衡其贡献度。
%
%贡献函数的目标是根据不同block的输入特征信息估计其特征的相关性。
%我们建立在最近的研究()上，这些研究表明卷积特征中的大部分信息是通过不同信道的统计及其相互依赖性来捕获的。
%我们只考虑通过全局平均汇集收集的渠道方式，即只考虑特征压缩为1×1×C通道描述符，所以直接在特征连接层进行贡献度的计算。
%为了捕获通道之间的依赖关系，我们添加了一个简单的非线性函数，它由两个完全连接的层连接，并与ReLU激活函数相连。此操作的输出是图层的贡献度分数。具体的。。。
%得到不同block输出特征的贡献度的分数后，将原本特征按照贡献度分数加权相加就是我们的基于atention的多尺度决策模块。
General CNNs conduct classification only based on the last fully-connected layer. 
However, in lightweight network, we must make full use of  the few features.  
High-level features focus more on the semantic meaning and low-level features are more about edge and texture.
For example, if we want to classify the dogs and cats, we should pay more attention on the high-level feature maps.
On the contrast, in classification of Persian Cat and American Shorthair, we should be more care about low-level features. 

Motivated by this idea, we use output features maps from all units to conduct classification, which called as Hierarchical Joint Decision, as illustrated in Fig. \ref{fig:attention}. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=.5\textwidth]{image/attention.pdf}
    \caption{Hierarchical Joint Decision based on Attention }
    \label{fig:attention}
\end{figure}

The most intuitive way of joint decision is that the feature maps of different units are directly connected for classification. 
This naive idea can only suitable for the same size  feature maps. 
However, through the consecutive downsampling operations in the network, feature maps from each unit vary in size.

% We also can downsample these feature maps into a fixed sizeto fuse them.
% However, this method also has a disadvantage: the feature maps obtained by downsampling has lost information which is unique to their level. It would lead to disturbance with the network classification \xu{add a reference to the experimental table}.

% This compresses the input features into 1 $\times 1 \times C$ channel (consider input feature maps is $H \times W \times C$)descriptor.
We build upon recent studies \cite{Hu2017SENet,Veit2017gata} which show that much of the information in convolutional features is captured by the statistics of the different channels and their dependencies\xu{not clear}.
Thus, we use the average pooling to compress the feature maps $X_{k} \in \mathbb{R}^{h \times w \times c_{k}}$  outputted from unit $k$  into one-dimensional vectors $Z_{k} \in \mathbb{R}^{1 \times 1 \times c_{k}} $  (Eq. \ref{equ:avg_pool}), and then directly connect all these one-dimensional features together.

\begin{equation}
Z_{k}=\frac{1}{h \times w} \sum_{i=1}^{h}\sum_{j=1}^{w} x_{i,j,c_k}
\label{equ:avg_pool}
\end{equation}

In addition, we noticed that feature maps from different units should be given different attention during joint decision making.  
In order to reflect the various importance of different hierarchical features, we endow the feature vectors with adaptive weights by means of attention mechanism.
% We add two fully-connected layers connected with a ReLU activation function on.
% The output of this operation is the importance score for different layer. 
% Specifically, it is a vector $\beta$ containing different scores for the $k$ units.
We add two fully-connected layers on the feature vector $Z_k$, whose output $\alpha
_{k}$ is the weight of attention. 
\begin{equation}
\alpha_{k}=W_2(\sigma(Z_{k}W_1))
\label{equ: ad_weight}
\end{equation}
\yang{not clear}
where $\sigma$ refers to the activation function ReLU, $W_1 \in \mathbb{R}^{ C_{k} \times d}$, $W_2 \in \mathbb{R}^{d \times 1}$ and $d$ is the dimension of the hidden layer.
The final classification layer can be computed according the Eq. \ref{eq:attention}, where $W_{cls}$ is weight of classification layer and $[\cdot]$ is concatenate operation.

\begin{equation}
\label{eq:attention}
pred=\mathbf{softmax}( W_{cls} \cdot   [\alpha_{1} Z_{1} ,..., \alpha_{k} Z_{k} ])
\end{equation}

% \begin{figure}
%     \centering
%     \includegraphics[width=.5\textwidth]{image/pre.pdf}
%     \caption{classification layer of Traditional CNN model.}
%     \label{fig:pre classification}
% \end{figure}



% The green module is the Composite Function  $\mathbf{H}$  operation.
% In our implementation, we use the bottleneck depth-separable convolution with inverse residuals in $\mathbf{H}$.
% The red lines indicate our proposed Exchange Shortcut Connection, from which show how we can achieve information interaction between groups without any additional computation. 
% The blue module denotes the achievement of Dense Funnel Layer.

% \subsubsection{Composite Function $\mathbf{H}$} 
% \label{H}
% Like introduction in \cite{Sandler2018MobileNetV2}, we define $\mathbf{H_l(\cdot{})}$ as a composite function of three consecutive operations:  a convolution operation(Conv),  a rectified linear unit (ReLU6) activation function \cite{Krizhevsky2012alexnet} and followed by batch normalization (BN) \cite{Ioffe2015Batch}.
% For the  convolution layer, we use a computational economical  $k \times k$ depthwise convolution \cite{Chollet2016Xception,howard2017mobilenets} based on the inverse residual bottleneck structure \cite{Sandler2018MobileNetV2}.


% For example, if we want to classify the dogs and cats, we should pay more attention on the high-level feature maps.
% On the contrary, in classification of Persian Cat and American Shorthair, we should be more care about low-level features. 


% Traditional convolutional feed-forward networks connect the output of the $l_{th}$ layer as input to the $(l+1)_{th}$ layer, which gives rise to the following layer transition: $\boldsymbol{X_{l}} = \mathbf{H} \left(  \boldsymbol{X_{l-1}}  \right)$.
% Based on this structure, ResNet \cite{he2016resnet} add a skip-connection that bypasses the non-linear transformations for avoiding the degradation problem as the depth of network increasing.


% If we divide all operations in this network into two groups, and conduct convolution respectively, these grouped network can be recursively defined.

% \begin{equation}
% \label{divide_resnet}
% \begin{aligned}
% &\boldsymbol{X}^1_{l-1},\boldsymbol{X}^2_{l-1}=\mathbf{Split}(\boldsymbol{X}_l)\\
% &\boldsymbol{ X}^1_{l} =  \mathbf{H}(\boldsymbol{X}^1_{l-1})+\boldsymbol{X}^1_{l-1}\\
% &\boldsymbol{ X}^2_{l} =  \mathbf{H}(\boldsymbol{X}^2_{l-1})+\boldsymbol{X}^2_{l-1}\\
% &\boldsymbol{ X}_{l} =[\boldsymbol{ X}^1_{l},\boldsymbol{ X}^2_{l}]
% \end{aligned}
%\end{equation}

% If we divide all operations in this network into two groups, we introduce \textbf{Exchange Shortcut Connection}, which can be recursively defined as Eq. \ref{exchange_resnet} to achieve the information interaction between different groups. 



 




==> image/001_introduction.tex <==
\section{Introduction}
\label{introduction}
Nowadays, Convolutional Neural Networks (CNNs) are widely applied in various computer vision tasks, including image classification~\cite{Krizhevsky2012alexnet,Huang2016ResNet}, object detection~\cite{Ren2015Faster}, face recognition~\cite{Taigman2014DeepFace,Liu2017SphereFace}, and style transfer~\cite{Gatys2016Image_stlye}, etc.
In order to achieve higher accuracy, modern CNNs tend to be equipped with hundreds of hidden layers and numerous training parameters \cite{Chollet2016Xception,Huang2016ResNet,Huang2016Densely}, resulting in enormous computation {\color{blue} loads} at billions of FLOPs (\textbf{Fl}oating-Point \textbf{Op}erations).
Therefore, training and deploying deep learning models are still difficult tasks which require plenty of computing resources and expensive hardwares such as GPU or TPU.

{\color{blue} On the other hand, considering the applications in practice, we urgently expect to deploy CNNs on embedded systems such as Internet-of-Things (IOT) devices, mobile phones, etc.,}{\color{red} rather than the large GPU server clusters or cloud platform. }
Those embedded systems suffer from the computation resource limitation so that the general state-of-the-art large CNN models, like ResNet \cite{he2016resnet} and VGGNet \cite{simonyan2014very}, are not applicable to them.
{\color{blue} For this reason, CNN models with satisfying accuracies under limited computational budgets (tens or hundreds of MFLOPs, i.e. Million Floating-Point Operations) are required for such resource-constrained scenarios.}

{\color{blue} In recent years, many researches focus on building lightweight and efficient neural networks, including Xception \cite{Chollet2016Xception}, MobileNet \cite{howard2017mobilenets}, MobileNetV2 \cite{Sandler2018MobileNetV2}, ShuffleNet \cite{Zhang2017ShuffleNet}, etc.
Through comprehensive survey on those studies, we have found that lightweight networks architecture tend to be shallow and thin for efficiency. }
{\color{red} Aiming to achieve satisfying accuracies in such networks, we must make full use of existing information resources of it.
Thus, different from the focus of lightweight networks design in the past, in this paper, we propose \textit{Super Interaction Network (SINet)}, which pays more attention to how to reduce the network scale by enhancing information interaction to increase the reusability of various features. }

We summarize the following contributions of SINet on how to achieve better information interaction with low computational complexity and parameters:
\begin{itemize}
\item We propose a novel group-based feature exchange method, named \textit{Exchange Shortcut Connection}. {\color{blue} All convolution operations of SINet are divided into multiple groups for computation reduction, and then we use exchange shortcut connections between groups to enhance the information interaction along the width of network. }
\item We propose \textit{Dense Funnel Layer}, which is equipped with dense connections like DenseNet \cite{Huang2016Densely}, but greatly reduces the computational cost to save memory resources. } It improves the information interaction along the depth of network.
\item For the final classification layer, we comprehensively exploit the usefulness of middle-layer features by means of the attention mechanism.  It improves the information interaction along the depth of network.
\item We conduct experiments on ILSVRC  2012 and CIFAR-100 datasets.
{\color{blue} We experimentally demonstrate the superiority of SINet compared with other state-of-the-art lightweight networks on benchmark datasets, including ILSVRC 2000, CIFAR-100 and ImageNet. } We also verify the effectiveness and universality  of our proposed components through ablation studies.

\end{itemize}






==> image/002_related_work.tex <==
\section{Related Work}
\label{related work}

\subsection{ Efficient Model Design}
There have been many works focused on the lightweight network design in recent years.
Two common basic components of these proposed models are \textit{group convolution} and \textit{channel integration}.

\subsubsection{Group convolution}
\label{Group convolution}
Group convolution can save the computational load by convolving on feature map groups respectively, rather than all feature maps outputted by the preceding layer.  It therefore becomes a standard component of lightweight networks.

Group convolution was first introduced in AlexNet \cite{Krizhevsky2012alexnet} for distributing the model over two GPUs to handle the memory explosion issue because of limited hardware resources.
After that, depthwise separable convolution was proposed in Xception \cite{Chollet2016Xception} and generalized the ideas of group convolutions in Inception series.
\cite{xie2017aggregated} proposed the concept of cardinality, which represents the group of channels.
Its model, ResNet, demonstrated the effectiveness of group convolution.
\cite{howard2017mobilenets} utilized channel-wise convolution and achieved the state-of-the-art results among lightweight models.
Channel-wise convolution is a special case of group convolution, where each group contains only one channel of feature maps.
Our SINet also utilizes group convolution through the network, but in a totally novel form.

\subsubsection{Channel Integration}
\label{Channel Integration}
Although group convolution can greatly reduce the computation of the network, it also leads to the information barrier among the groups because each group is independently convoluted .

To deal with this problem, modern CNN library \textit{Cuda-Convnet} supported ``random sparse convolution'' layer, which implemented random channel shuffle after group convolutional layer.
IGC \cite{Zhang2017IGCV,Xie2018IGCV} adapted permutation operation for a two-stage convolution in order to mix the different group features.
MobileNet \cite{howard2017mobilenets} leveraged the point-wise convolution after channel-wise convolution to reintegrate the separated channels.
ShuffleNet \cite{Zhang2017ShuffleNet,Ma2018ShuffleNet} proposed the channel shuffle operation for grouped point-wise convolution.
Different from the previous studies, in this paper, we introduce a novel operation, named Exchange Shortcut Connection, which can be used to share the information between different groups. 
Most importantly, it needs no extra computation at all.

\subsection{Network Design and Shortcut Connection}

Empirically speaking, in order to obtain a more effective network, an intuitive and naive extension method is increasing the depth of neural networks \cite{simonyan2014very}, such as AlextNet~\cite{Krizhevsky2012alexnet}, ZF-Net~\cite{Matthew2013ZFNet} and VGGNet~\cite{simonyan2014very}.
However, as the depth of  network increases, the gradient back propagation becomes more and more difficult, and the gain obtained by simply increasing depth  tends to be saturated.
ResNet \cite{he2016resnet} proposed a simple identity skip-connection to ease this issue of the deep networks.
Based on the skip-connection  architecture, various models such as WideResNet \cite{zagoruyko2016wideresnet}, Inception-ResNet \cite{szegedy2017inception4}, and ResNeXt \cite{xie2017aggregated} have been developed.
Recently, DenseNet \cite{Huang2016Densely} proposed a new architecture ---\textit{ Dense Connection} which iteratively concatenates the input features with  the output features so that each convolution unit can receive raw information from all preceding units.
In this paper, we borrow the idea from the skip-connection and DenseNet to improve the accuracy and efficiency of networks.

\subsection{Attention Mechanism}
As introduced in \cite{Hu2017SENet}, attention can be interpreted as a method of biasing the allocation of available computational resources towards the most informative components of a signal.
{\color{blue} Implementations of the attention mechanism can be categorized into two classes: soft attention that keeps all components weighted, and hard attention that selects a part of components with a certain sampling strategy. }

In recent years, attention mechanism have been applied to a variety of practical tasks and  proven to be very effective.
These tasks include:
image caption \cite{chen2017sca,lu2017knowing}, machine translation \cite{luong2015effective,bahdanau2014neural}, localization \cite{Olga2015ImageNet} and understanding in images\cite{chen2017sca}.
There also have been many attempts \cite{Hu2017SENet} to incorporate attention mechanism for improving the accuracy in classification tasks.
Residual Attention Network~\cite{wang2017residualattention} proposed an encoder-decoder style attention module.
By refining feature mapping, the network not only works well, but also is robust to noise.
SENet \cite{Hu2017SENet} introduced Squeeze-and-Excitation module, which used the global average summarization feature to calculate channel attention.
 %a compact module to take advantage of the inter-channel relationship.

By contrast, our proposed Hierarchical Joint Decision based on Attention in our lightweight model focuses on how to exploit the features of middle layer for final classification.




==> image/003_model.tex <==
\section{Model}
\label{approach}
In this section, we propose three new operations applied in SINet, including  Exchange Shortcut Connection, Dense Funnel Layer and
Attention based Hierarchical Joint Decision.
After that, we illustrate the overall architecture of SINet.

\subsection{Exchange Shortcut Connection}
\label{Exchange Shortcut Connection}

As mentioned in Sec.~\ref{Channel Integration}, the group convolution operation is a commonly used method in lightweight models.
However, although group convolution can save the computation cost, it is obvious that the information interaction between groups is completely interrupted because outputs from a certain group are only related to its own inputs, like shown in Fig.~\ref{fig:group}.

\begin{figure}[h]
\centering
\includegraphics[height=.29\textwidth]{image/Block2.pdf}
\caption{Group convolution. Feature maps with different colors (blue and green) represent  different groups. Convolution operations are performed independently on both groups.}
\label{fig:group}
\end{figure}

{\color{blue} Many models have been proposed deal to with this intractable problem, but they require extra structures and computations to mix up separated groups.}
For example, in MobileNet, the proposed point-wise convolution for channel reintegration occupies 93.4\% computation of the network \cite{howard2017mobilenets}.

Different from previous works, in SINet, we propose a totally novel and more efficient method, named \textit{Exchange Shortcut Connection}, which can achieve the information interaction among groups without any extra computation.

\begin{figure}
\centering
\includegraphics[width=.45\textwidth]{image/Block1.pdf}
\caption{The detail of operations in SI Units, where the red bold lines denote the Exchange Shortcut Connections. \textbf{C} denotes concat operation and \textbf{DF} denotes Deep Funnel Layer.}
\label{fig:group and exchange}
\end{figure}

We define $\mathbf{H}(\cdot)$ as a composite convolution function, and let $\mathbf{H}_l(\cdot), l \in {1, ..., N}$ denote the convolution function computed by the $l_{th}$  layer.
 $\boldsymbol{X_{0}}$ represents input image and $\boldsymbol{X_{l}}$ is output of the $l_{th}$ layer.
Inspired by ResNet \cite{he2016resnet}, whose standard shortcut connection can be recursively defined as: $\boldsymbol{X_{l}} = \mathbf{H}\left ( \boldsymbol{X_{l-1}} \right )+\boldsymbol{X_{l-1}}$, if we divide convolution operations in our network into two groups, Exchange Shortcut Connection can be recursively defined as Eq. \ref{exchange_resnet}, where $[\cdot]$ means the concat operation.
\begin{equation}
\label{exchange_resnet}
\begin{aligned}
&\boldsymbol{X}^1_{l-1},\boldsymbol{X}^2_{l-1}=\mathbf{Split}(\boldsymbol{X}_l)\\
&\boldsymbol{ X}^1_{l} =  \mathbf{H}(\boldsymbol{X}^1_{l-1})+\boldsymbol{X}^2_{l-1}\\
&\boldsymbol{ X}^2_{l} =  \mathbf{H}(\boldsymbol{X}^2_{l-1})+\boldsymbol{X}^1_{l-1}\\
&\boldsymbol{ X}_{l} =[\boldsymbol{ X}^1_{l},\boldsymbol{ X}^2_{l}]
\end{aligned}
\end{equation}
Fig.~\ref{fig:group and exchange} illustrates two stacked group convolutions with Exchange Shortcut Connection.
Compared with Fig.~\ref{fig:group}, Exchange Shortcut Connection allows different convolution groups to access input data from others, which builds up information interaction among groups.
We emphasize that this method needs no extra computational cost and can be easily and flexibly extended to other existing architectures.

Compared with general CNNs, our structure can achieve less computation complexity under same settings.
{\color{blue} Given a convolution operation with the kernel size $k \times k$, when the input size is $c \times h \times w$ and the output channels number is $m$, general convolution requires $c \times h \times w \times k \times k \times m$ FLOPs, while our proposed unit only requires $c \times h \times w \times k \times k \times m / g$ FLOPs, where $g$ denotes the number of groups. }

\subsection{Dense Funnel Layer}

\subsubsection{Dense Funnel Layer}
\label{dense funnel layer}

Traditional shortcut connections \cite{he2016resnet} only leverage the information of the nearest preceding layer.
To further improve the information interaction along the depth of network, we expect to connect the current layer with all preceding layers, like DenseNet \cite{Huang2016Densely}.

{\color{blue} Although these dense connections have been proven to be very effective in general CNNs model, they would obviously cause a explosive growth of memory and computation cost, which is not acceptable for a lightweight network.}
Thus, we introduce a novel structure called \textit{Dense Funnel Layer}.

Fig.~\ref{fig:narrow} schematically illustrates the layout of Dense Funnel Layer.
The different colored lines in the figure represent the data flows of different layers.
The green boxes indicate the first set of feature maps at the beginning, and the orange boxes are the feature maps obtained after the composition convolution operation $\mathbf{H}$ applied on green feature maps.


\begin{figure*}[h!]
\centering
\includegraphics[height=.18\textwidth]{image/narrow.pdf}
\caption{A 3-layer Block with Dense Funnel Layer. Where $\mathbf{H}$ indicates Composite function, $\mathbf{DF}$ indicates Dense Funnel Layer and $\mathbf{C}$ indicates concat operation.}
\label{fig:narrow}
\end{figure*}

Firstly, we combine features from preceding convolution layers (green feature maps \RNum{1}) and current layer output features (red feature maps \RNum{2}) by concatenating them.
{\color{blue} Then we use a $1\times 1$ convolution layer to reduce the channels and mix the information from both sources, getting the output feature maps \RNum{3}. 
This operation is the key for avoiding the explosive growth of memory cost caused by the dense connection, because it squeezes out the useless information of the preceding feature maps}.
After that, we feed these mixed feature maps to the next layer and conduct the the similar operations repeatedly {\color{red} (connect green, orange and purple feature maps, apply $\mathbf{H}$ and Dense Funnel layer on them)}.
After several iterations in the network, we can hold a view that the last set of feature maps approximately contains the information of all preceding feature maps .

\subsection{Attention based Hierarchical Joint Decision}
\label{attention decision}
High-level features focus more on the semantic meaning and low-level features are more about edge and texture.
General CNNs conduct classification only based on the last layer of the network which belongs to the high-level features.
Aiming to making full use of {\color{blue} all } features in the lightweight network, we utilize the outputs from all middle layers which contain high and low level features to conduct classification. 
We call it as \textit{Attention based Hierarchical Joint Decision}, like illustrated in Fig. \ref{fig:attention}.

\begin{figure}[h]
\centering
\includegraphics[width=.5\textwidth]{image/attention.pdf}
\caption{Attention based Hierarchical Joint Decision.}
\label{fig:attention}
\end{figure}
The most intuitive way of joint decision is that the feature maps of different layers are directly connected for classification.
This naive idea is only suitable for same sized feature maps.
% \yang{C}
{\color{blue} However, through the consecutive downsampling operations in the network, if each {\color{red} Block } only contains one downsampling operation, then feature maps from all red Blocks} vary in size. }

We build upon recent studies \cite{Hu2017SENet,Veit2017gata} which show that much of the information in convolutional features is captured by the statistics of the different channels and their dependencies.
Thus, we use the average pooling to compress the feature maps $X_{k} \in \mathbb{R}^{h \times w \times c_{k}}$  outputted from Block $k$  into one-dimensional vectors $Z_{k} \in \mathbb{R}^{1 \times 1 \times c_{k}} $: 
\begin{equation}
Z_{k}=\frac{1}{h \times w} \sum_{i=1}^{h}\sum_{j=1}^{w} x_{i,j,c_k},
\label{equ:avg_pool}
\end{equation} 
and then connect all these one-dimensional features together.

In addition, we notice that the feature maps from different Blocks should be given different attention during joint decision making.
In order to reflect the various importance of different hierarchical features, we endow the feature vectors with adaptive weights by means of attention mechanism.
We add two fully-connected layers on the feature vector $Z_k$, whose output $\alpha_{k}$ is the weight of attention, like shown in Eq.~\ref{equ: ad_weight}.
We expect the network to automatically learn how to assign the attention to different feature maps from each level.
\begin{equation}
\alpha_{k}=\sigma((Z_{k}W_{1})W_{2})
\label{equ: ad_weight}
\end{equation}

In Eq. \ref{equ: ad_weight},  $\sigma$ refers to the sigmoid activation function , $W_1 \in \mathbb{R}^{ C_{k} \times d}$, $W_2 \in \mathbb{R}^{d \times 1}$ and $d$ is the dimensionality of the hidden layer.

The final classification layer can be computed according to Eq. \ref{eq:attention}, where $W_{cls}$ is the weights of classification layer and $[\cdot]$ is concat operation.

\begin{equation}
\label{eq:attention}
pred=\mathbf{softmax}( W_{cls} \cdot   [\alpha_{1} Z_{1} ,..., \alpha_{k} Z_{k} ])
\end{equation}

\subsection{Architecture }

\subsubsection{SI Unit and SI Block}
\label{si unit}

Taking advantage of the \textit{Exchange Shortcut Connection} and \textit{Dense Funnel Layer} operations, we propose \textit{SINet Unit} which can be seamlessly embedded into {color{blue} other existing CNN networks} and the amount of network {color{blue} computation } can be greatly reduced with less accuracy decline.

An SI Unit is composed of 3 basic computing operations, including Exchange Shortcut Connection, Composite Convolution Function  $\mathbf{H}$ and Dense Funnel Layer, as illustrated in Figure \ref{fig:group and exchange}.

$\mathbf{H}$ consists of a convolution operation~(Conv),  a rectified linear unit (ReLU6) activation function \cite{Krizhevsky2012alexnet}, and followed by batch normalization (BN) \cite{Ioffe2015Batch}.
For the convolution layer, we use a computationally efficient $k \times k$ depthwise convolution \cite{Chollet2016Xception,howard2017mobilenets} based on the inverse residual bottleneck structure \cite{Sandler2018MobileNetV2}.

\begin{figure*}[h!]
\centering
\includegraphics[width=\textwidth]{image/exchange.pdf}
\caption{An SI Block with 3 SI Units. \textbf{ S} indicates split operation which divides the input feature maps into $g(g=2)$ groups,\textbf{ M} indicates Merge operation which connects the feature maps of different groups and \textbf{C} indicates concat operation in the exchange shortcut.}
\label{fig:exchange units}
\end{figure*}

\textit{SI Block} in our network is formed by a stack of \textit{ SI Units} which can achieve fully information interaction of the different groups and different units, like shown in Fig \ref{fig:exchange units}.
Several SI Blocks are stacked together to form the entire network.

\subsubsection{Network Architecture Overview}
{\color{blue} Built on SI Units, SI Blocks and Hierarchical Joint Decision, we present the overall SINet architecture in Table \ref{tab:overall architecture}. 
Similar to MobileNetV2, the architecture of SINet can be customized to meet the requirements of accuracy/performance trade-offs through the \textit{width multiplier} parameter $w$. }
As $w$ becomes larger, the network suffers from more parameters and computational overhead, but it can achieve higher accuracy.

\begin{table}[h]
\footnotesizexq
  \centering
  \caption{SINet architecture. Each Block describes a sequence of identical layers, repeated $n$ times. $k$ denotes the kernel size. All layers in the same sequence have the same number of output channels. The first layer of each sequence has a stride $s$ and all others use stride 1. The expansion factor $t$ is the multiplying factor of inverse residual convolution introduced in \cite{Sandler2018MobileNetV2}, and $w$ is width multiplier.}
  \vspace{5}
    \begin{tabular}{c|c|c|c|c|c|c}
    \toprule
    Layers & output & $k$ & s & $n$ & $t$     & operator \\
    \midrule
    Image & 224^2 \times 3 &       &       &       &       &  \\
    \midrule
    Block1 & 112^2 \times (24 \cdot w) & 3 \times 3    & 2     & 4     & 3     & bottleneck \\
    \midrule
    Block2 & 56^2 \times (40 \cdot w) & 5 \times 5    & 2     & 4     & 3     & bottleneck \\
    \midrule
    Block3 & 28^2 \times (80 \cdot w) & 5 \times 5    & 2     & 4    & 6     & bottleneck \\
    \midrule
    Block4 & 14^2 \times (96 \cdot w)  & 3 \times 3    & 2     & 4    & 6     & bottleneck \\
    \midrule
    Block5 & 7^2 \times (192 \cdot w) & 5 \times 5    & 2     & 4    & 6     & bottleneck \\
    \midrule
    \multirow{3}[2]{*}{Decision} & 1^2 \times (432 \cdot w) & 7\times 7     &       & 1     &       & \multicolumn{1}{l}{avg pool} \\
    \cmidrule{2-7}
          & 1^2 \times 1280 & 1 \times 1    &       & 1     &       & fc \\
     \cmidrule{2-7}
          & 1^2 \times c & 1\times 1     &       & 1     &       & fc \\
    \bottomrule
    \end{tabular}%
  \label{tab:overall architecture}%
\end{table}%

The architecture of SINet contains a initial fully convolution layer with 21 filters, followed by 5 SI Blocks.
The convolution operation for each  SI Block is performed in two groups, and the first SI Unit of each  SI Block is always applied with stride = 2 in $k \times k$ Conv for down sampling.
In the final decision layer, we apply the Hierarchical Joint Decision based on Attention operation on all output feature maps from all SI Blocks.
Then we add a fully-connected softmax layer on it for classification.



==> image/004_experiment.tex <==
\section{Experiment}
\label{experiment}
In this section, we evaluate the effectiveness of SINet through a series of experiments.
Firstly, we exhibit the high accuracy and efficiency of SINet on ImageNet ILSVRC 2012 classification task.
Secondly, we also show the validity and universality of our purposed components by means of Ablation Studies on CIFAR-100 dataset.
\subsection{Image Classification on ImageNet}
\subsubsection{Training setup}
\label{dataset:imagenet}
The ILSVRC 2012 classification dataset consists 1.28 million images for training, and 50,000 for validation, from 1000 different classes.
We train networks on the training set and report the top-1 and top-5 accuracy on the validation set.
We train our models using Pytorch, and optimization is performed using synchronous SGD with momentum $0.9$ and batch size of $256$.
Following MobileNet \cite{howard2017mobilenets,Sandler2018MobileNetV2} setup, we use initial learning rate of 0.045, and learning rate decay rate of 0.98 per epoch.

\subsubsection{Results}
We compare our SINet with several state-of-art networks on the ImageNet dataset.
The specific statistics of different models and their accuracy can be seen in Table \ref{tab:imagenet}.

Firstly, compared with some general non-lightweight models,  our SINet can achieve comparable accuracy but only requires about 1/55 FLOPs of VGG-16 and 1/6 FLOPs of ResNet-34.
Secondly,  SINet outperforms the state-of-art lightweight models (including MobileNets and ShuffleNets) under much lower computation cost.
Finally, we also compare SINet with the models generated by different strategy, such as AutoML and Pruning technology.
NASNet~\cite{Zoph2017nasnet} is the deep networks automatically searched using reinforcement learning model.
CondenseNet~\cite{Gao2017CondenseNet} is an efficient CNNs architecture which encourages feature reuse and prunes filters associated with superfluous features.
{\color{blue} SINets can even achieve higher accuracy than them with comparable amounts of FLOPs and parameters, but does not need assistance from extra strategies. }
\begin{table}[h]
\footnotesize
  \centering
  \caption{ImageNet comparative experiment results.}
    \begin{tabular}{l|rccc}
    \toprule
    Model   & \multicolumn{1}{c}{Params} & FLOPs & Top1(\%) & Top5(\%)  \\
    \midrule
    VGG-16 & \multicolumn{1}{c}{15.2M} & 1535M     & 71.93    & 90.67     \\
    ResNet-34 & \multicolumn{1}{c}{22.8M} & 3580M     & 74.97      & 92.24      \\
    \midrule
     AlexNet &     \multicolumn{1}{c}{6.1M}     & 720M    & 62.5    & 83.0      \\
    SqueezeNet & \multicolumn{1}{c}{3.2M} & 708M     & 67.5    & 88.2     \\
    MobileNetV1 & \multicolumn{1}{c}{4.2M} & 575M     & 70.6    & 89.5     \\
    MobileNetV2 & \multicolumn{1}{c}{3.6M} & 322M     & 71.8      & 91.0       \\
    MobileNetv2(1.4) & \multicolumn{1}{c}{6.9M} & 585M     & 74.7    & 92.5    \\
    ShuffleNet(1.5) & \multicolumn{1}{c}{3.4M} & 292M    & 71.5    & -        \\
    ShuffleNet(\times2) & \multicolumn{1}{c}{5.4M} & 524M     & 73.7    & -         \\
    ShuffleNetv2(2\times) & \multicolumn{1}{c}{-} & 591M    & 74.9   & -        \\
    \midrule
    \scriptsize{CondenseNet(G=C=4)} & \multicolumn{1}{c}{2.9M} & 274M     & 71.0      & 90.0      \\
   \scriptsize{CondenseNet(G=C=8)} & \multicolumn{1}{c}{4.8M} & 529M     & 73.8    & 91.7    \\
   NASNet-A & \multicolumn{1}{c}{5.3M} & 564M     & 74.0      & 91.3    \\
    \midrule
    SINet(1.0)   &  \multicolumn{1}{c}{ 3.0M}        &   208 M      &  70.1         &  89.4        \\
    SINet(1.2)   &    \multicolumn{1}{c}{ 3.9M}      &  280M       &   71.0      &  90.0       \\
    % SINet(1.4)   &    \multicolumn{1}{c}{ 4.8M}      &  368M       & \change{72.1}        &  \change{90.5}        \\
    SINet(1.6)   &    \multicolumn{1}{c}{ 6.0M}      &  468M       & 73.1        &  91.0       \\
    SINet(1.8)   &    \multicolumn{1}{c}{ 7.6M}      &  570M       & 74.8         &    92.6      \\
    \bottomrule
    \end{tabular}%
  \label{tab:imagenet}%
\end{table}%

\subsection{Ablation Studies}
\label{ablation}
The core idea of our proposed SINet lies in SI Units and Hierarchical Joint Decision based on Attention.
In order to verify the universality and effectiveness of both components, we apply them to 4 different existing models (including two lightweight models and two general CNN models) and compare their accuracy respectively.
For fair comparison, we use the standard implementation of these existing models described in corresponding papers \cite{howard2017mobilenets,Sandler2018MobileNetV2,Ma2018ShuffleNet,Hu2017SENet}.
We also compare the computation cost of these existing models under different setup.
Following the general testing protocol, we report the computational cost by counting the total number of the Multiply-Add operations and  parameters under the standard ImageNet dataset input size ($224 \times 224$).
\subsubsection{Training setup}
The CIFAR-100 dataset consists of colored natural images with $32 \times 32$ pixels.
The training and testing sets contain 50000 and 10000 images, respectively.
We train networks on the training set and report the accuracy on the testing set.

We train all models using Pytorch and optimize them using synchronous SGD with momentum $0.9$ and batch size of $128$.
All models are trained for 150 epochs from scratch.
The initial learning rate is set to $0.01$ and decreased by a factor of 10 every 80 epochs.

\subsubsection{SI Unit}
In order to verify the effectiveness of the SI Unit, we compare the original networks \textbf{A} without group convolution ($G=1$), the networks \textbf{B} that only use group operation ($G=2$) but no shortcut exchange connection (EX=No), and the networks \textbf{C} that utilize the SI Unit, including both of group convolution  and shortcut exchange connection ($G=2$, EX=Yes) in our experiment.
For fairness, we use exactly the same settings to train these models.
Results are shown in Table \ref{tab:exchange unit}.

% % exchange unit
\begin{table}[h]
\footnotesize
  \centering
  \caption{SI Unit under different networks architecture.
 {\color{blue} $G$ denotes the number of groups, and $EX$ denotes whether to use Exchange Shortcut Connection.}}
    \begin{tabular}{c|ccccc}
    \toprule
    Model   & $G$       & $EX$      & Params(M) & FLOPs(M) & Acc.(\%) \\
    \midrule
    \multirow{3}[1]{*}{MobileNet} & 1       & -       & 4.23    & 575.00     & 74.33    \\
            & 2         & Yes       & 2.66    & 291.55  & 75.51    \\
            & 2        & No       & 2.66    & 291.55  & 73.95    \\
    \midrule
    \multirow{3}[1]{*}{MobileNetv2} & 1       & -       & 3.56    & 322.47  & 71.59    \\
            & 2    &Yes       & 2.89    & 224.38  & 71.71    \\
            & 2        & No       & 2.89    & 224.38  & 70.74    \\
    \midrule
    \multirow{3}[1]{*}{ResNet34} & 1       & -       & 21.79   & 3579.76 & 75.90    \\
            & 2       & Yes      & 12.99   & 2109.00    & 74.35   \\
            & 2       & No      & 12.99   & 2109.00    & 73.22   \\
    \midrule
    \multirow{3}[1]{*}{SENET} & 1       & -       & 11.79   & 1730.16 & 75.77   \\
           & 2       & Yes      & 7.37    & 978.68  & 75.23    \\
           & 2        & No      & 7.37    & 978.68  & 73.80     \\
    \bottomrule
    \end{tabular}%
  \label{tab:exchange unit}%
\end{table}%

From the results, we see that the networks \textbf{B} which only use group operation can greatly reduce the parameter and computation, but at the same time, its accuracy is lower than that of original network \textbf{A} in all four network architecture.
The network \textbf{C} using the SI Unit can achieve the same amount of parameters and computational complexity as the network \textbf{B} while maintaining a satisfying accuracy compared with the original network \textbf{A}.
Especially in lightweight  networks (MobileNet V1 and V2), the networks \textbf{C} using the SI Unit even obtain better results than that of  original network \textbf{A}.
It shows that the design of SI Unit compensates for information blocking due to the use of group convolution.
In addition, it also manifests that the information interaction in shallow networks is more important than that in deep networks.

\subsubsection{Hierarchical Joint Decision based on Attention }
In order to verify the validity of the Hierarchical Joint Decision based on Attention {\color{red} (JDA Layer for short)}, we compare the original networks \textbf{A} which use general classification layer (JDA=No) and the networks \textbf{B} that utilizes the JDA Layer (JDA=Yes) in our experiment.
{\color{blue} We use the same settings as the former experiment to train these models.}
Results are shown in Table \ref{tab:attention cifar100}.
% Table generated by Excel2LaTeX from sheet 'Sheet4'
\begin{table}[h]
\footnotesize
  \centering
  \caption{JDA Layer under different networks architecture.}
    \begin{tabular}{c|cccc}
    \toprule
    Model   & JDA      & Params(M) & FLOPs(M) & Acc.(\%) \\
    \midrule
    \multirow{2}[1]{*}{MobileNet} & No       & 4.23    & 567.72  & 74.33 \\
           & Yes       & 5.24    & 567.72  & 74.66 \\
    \midrule
    \multirow{2}[1]{*}{MobileNetv2} & No       & 3.56    & 322.47  & 71.59 \\
            & Yes       & 2.43    & 322.47  & 73.24 \\
    \midrule
    \multirow{2}[1]{*}{ResNet34} &No       & 21.79   & 3579.76 & 74.48 \\
            & Yes       & 22.32   & 3579.76 & 76.06 \\
    \midrule
    \multirow{2}[1]{*}{SENET} & No       & 11.79   & 1730.16 & 75.45 \\
            & Yes       & 12.30    & 1730.16 & 75.10 \\
    \bottomrule
    \end{tabular}%
  \label{tab:attention cifar100}%
\end{table}%


{\color{blue} We can see that networks \textbf{A} using JDA layer consistently achieve better performance than original networks \textbf{B}, at the cost of a small amount of additional computations. }

It shows that the JDA layer which combines the output features of all middle blocks for joint decision is effective. It demonstrates that effective information interaction  along depth direction is necessary.


































==> image/005_conclusion.tex <==
\section{Conclusion}
\label{conclusion}
{\color{blue}
In this study, we introduce a novel light-weight convolutional neural network named SINet. 
SINet uses group convolution to reduce computational cost, and Exchange Shortcut Connections to share information between groups.
We also propose Attention based Hierarchical Joint Decision to make full use of all feature maps learned by convolutional layers.
%It is s simple network architecture that allow us to build a highly efficient litter models.
SINet allows very memory-efficient inference and relies utilize standard operations present in all neural frameworks.
Through experiments on the ImageNet dataset, we demonstrate that outperforms state-of-the-art light-weight models and widely-used full-sized networks like VGG-16.
Ablation studies on the CIFAR datasets verifies the universality of the newly designed components in SINet.
}

==> trash <==


% The rest of paper is organized as follows.
% Section \ref{related work} presents the related work.
% Section \ref{approach} introduces the proposed algorithm in our network.
% Section \ref{architecture} introduces the designed architecture.
% Section \ref{experiment} presents the empirical studies.
% Section \ref{conc} finally concludes the paper.


% These related approaches can be categorized into two classes: the first way is compressing existing large networks, the second is designing and training a lightweight network directly.
% The first class is the most commonly-used approaches including pruning\cite{Gordon2017FluidNets}, compressing\cite{Han2015Deep}, and low-bit representation\xu{need double check}\cite{Jacob2017Quantization}.
% The second direction focuses on lightweight network architectures design and better speed-accuracy trade-off, including Xception \cite{Chollet2016Xception}, MobileNet \cite{howard2017mobilenets}, MobileNetV2 \cite{Sandler2018MobileNetV2} ShuffleNet \cite{Zhang2017ShuffleNet}, etc. 


%首先，分组卷积引起了人们的注意，因为它在保持准确性的同时大大降低了计算复杂度，残差结构的设计减轻了深度网络的梯度下降现象，也增强了前后层的特征利用。
%我们在每一个block内部的特征计算中都将使用group convolution，但是考虑到组卷积组间信息不流通的特性，我们从残差结构中skip connect的设计出发，设计了一种新颖的exchange shortcut残差结构，来保证组间的信息交互。
%众所周知，组卷积等效于具有稀疏内核的常规卷积：不同分区中的信道之间没有连接。因此，exchange块等效于将不同分区之间的信道产生连接。
%我们表明，在相同数量的参数/计算复杂度下，基于exchange的分组块比常规卷积宽。我们还观察到，在相同的计算复杂度和相同数量的参数下堆叠具有exchange层的分组块构建的网络比具有常规分组卷积的网络表现更好。
%
%其次，每一个unit内部的block之间我们采用的是dense funnel的方式，每一个block将会接受来自当前unit中前面所有层信息，这些信息将会进行一步挤压操作后输入给当前block。
%
%最后，Attention based hierarchical joint decision我们使用来代替传统决策层，综合利用cnn网络计算中不同尺度（级别）的特征信息进行联合决策。我们观察到联合决策的方式要比传统的决策方式的网络表现更好。
%无论是手工设计网络结构，还是自动设计网络结构，现在的各种网络设计都要基于新颖有效的模块设计，特别是有效的轻量化结构。
%所以我们的目标一开始就是设计一系列独立的热插拔的各种模块，我们发现我们设计的各种模块可以根据网络设计的需要灵活使用。

% Firstly, grouped convolution has attracted attention because it reduces the computational complexity greatly while maintaining accuracy.
% The design of the residual structure mitigates the gradient degradation of the deep network and enhances the feature utilization of front layer.
% Group convolution we will used in the feature calculation of each block, but considering the non-circulation characteristics of the group convolution group, we design a novel \textit{Exchange Shortcut} from the design of skip connect in the residual structure to ensure information exchange between groups.
% As is well known, a group convolution is equivalent to a
% regular convolution with sparse kernels: there is no connections across the channels in different partitions.
% Therefore, \textit{Exchange} is equivalent to generating a connection between channels between different partitions.
% We show that under the same number of parameters/computational complexity, the Exchange-based block is wider than the conventional convolution. 
% We have also observed that a network constructed by stacking block group convolution with \textit{Exchange} under the same computational complexity and the same number of parameters performs better than a network with conventional group convolution.

% Secondly, \textit{Dense Funnel Layer} will be used between the blocks in each unit. 
% The information will direct transfer from any block to all subsequent blocks, and the connecting information will be squeezed and input to the current block.

% Finally,  \textit{Attention based Hierarchical Joint Decision} which comprehensively utilize different scales feature information will be used to replace the traditional decision layer.
% We observe that the network with joint decision performance better than traditional decision method.

% Group convolution and depth-wise convolution can be regarded as the crucial component in these works.
% Grouped convolution has attracted attention because it reduces the computational complexity greatly while maintaining accuracy.
% In this paper, we propose a $branch$ mechanism which is similar with group operation, and come up with a novel $exchange$ operation to help the information flowing between different groups to overcome the side effects brought by group convolutions --- Combined is $Branch and Exchange$.

% Successfully adopte in \cite{Huang2016ResNet}, skip connection is an efficient way to make top layers accessible to the information from bottom layers.
% To further activate the gradient and information flow in networks, DenseNet \cite{Huang2016Densely} proposed make any layer in a block is the output of all preceding layers, and the input of all subsequent layers.
% Recent studies show the effectiveness of activating information flow.
% Inspired by the maximum information flow and the inverted residual, we design a \textbf{narrow channel connection} structure.

% The design and development of new CNN architectures is a difficult engineering task, typically a new lightweight module.
% Designing a block which can be used directly in existing state-of-the-art architectures by replacing components with designed counterparts and can get desirable performance is looming which is our intent.

%最近，出现了许多专注于构建轻量级和高效神经网络的文献，包括Xception，MobileNet，MobileNetV2, ShuffleNet等,他们主要关注于如何。
%综合研究小型网络，我们发现小型网络一般较浅，为了在这样一个非极深层的网络中实现好的网络表现力，我们必须要充分利用现有的信息资源。
%因此，不同于以往小型网络工作的关注点，我们更多地关注如何通过增强信息交互来增加网络中功能的可重用性来减小网络规模。

% They replaced the first pointwise convolution layer with the pointwise group convolution followed by a channel shuffle operation.  
% However, IGCV1 \cite{Zhang2017IGCV} did not specially investigate the effectiveness of channel permutation itself and its usage in lightweight model design,
%  ShuffleNet \cite{Zhang2017ShuffleNet} did specially investigate the effectiveness of 1 × 1 layer or specific layers.\yang{need to change}
%他们更加关注于将来自不同组的信道打乱后进行重新分配，而不是将不同组的信息进行充分的交换。
% Instead of having a full interaction between the channel information of different groups, they are more concerned with shuffling channels from different groups and redistributing the distorting information.

 %现在的卷积神经网络通常由具有相同结构的重复构建块组成。其中，state-of-the-art的网络比如resnet，resneXt，mobilenet，shufflenet等使用depthwise separable卷积块堆叠而成，mobilenetv2使用了depthwise separable with inverted residual structure作为重复构建快等等，他们都是将有效的群组卷积或深度可分离卷积（也可以看作组卷积）引入构建块，以在表示能力和计算成本之间取得良好的折衷。
    %组卷积是最为简单使用的通道稀疏连接方式，所以被广泛利用，如公式所示，可以看出他可以将一个卷积层计算量降至原来的。。。倍。。
    %但是，组卷积堆栈具有明显的副作用：来自某个组的输出仅来自一小部分输入通道，这个属性阻止不同组之间的信息流并削弱表示特征。（见图）
    %shufflenet提出channel shuffle的思想，igcv2提出交错组卷积的思想，他们的目的都是为了打乱使用在point convolution上组卷积造成的信息不流通。
    %不同于这种专门设计用在单一卷积层上的组卷积操作，我们直接从输入特征图开始进行分组的计算，如图（）所示。
    %也不同于他们使用打乱信息——shuffle and permutation的方式来解决组间信息不流通的问题，我们提出一种新形的基于short connect的组间信息交互策略——Interaction。
    %short connect最早在resnet和高速公路网络中被提出用来降低随着网络深度的增加造成的梯度消失现象，其公式表示如下：
    %在我们的设计中，我们使用的short connect的另外一个主要功能：提高信息的交互。
    %首先是利用short connect来进行组间的信息交互，从图以及公式中可以明显的看出不同分支的计算操作互不干涉，某一分支的输出仅与该分支内的输入有关。我们提出的这种新型的基于分组计算的shortconnect操作的形式如图所示，不同于以往的旁支直连操作（。。），我们的计算操作如公式所示。（其中黑体表示不同）。
    
    
   %为了解决这个棘手的问题，MobileNetV1和MobileNetV2在depth-wise 卷积后利用逐点卷积重新集成了分离的通道。
    %由于逐点卷积占据93.4％计算，shufflenet和igcv在逐点卷积中使用群组卷积。 ShuffleNet引入了渠道混洗操作来混合各组之间的信息，IGCV2 提出了Interleaved Group Convolutions，打破了群体之间的障碍。
    
    
      %resnet中旁支直连的操作是为了可以利用到上一层的信息，那么为了可以进一步的利用信息，我们希望不仅仅可以使用到上一层的信息，我们希望可以利用到同一层级中前面所有层的信息.但是直接的connect操作，类似于densent中的dense connect会导致内存使用以及计算量的爆炸，densnet验证了denseconnect的有效性，但是很明显，这种操作无法实现轻量化的网络。
    %因此，我们引入了一种称为窄型全连接结构的新型连接结构。图说明了这种结构。
    %我们通过concat操作来组合当前层先前卷积块的所有特征（不同颜色的特征块，表示不同block产生的特征）。因此，l层有l-1个输入，图中的不同颜色的连接线表示不同特征的数据流。
    %首先是第一层信息的产生，绿色表示本组第一层计算所得的特征图，红色特征是经过卷积计算操作（H）后得到的特征，紫色特征块同理。使用shortcut连接方式，将本block内部前面所有一层信息于本层信息进行connect连接，为了避免 connect带来的内存计算量爆炸现象，使用narrow操作对concat后的特征进行挤压，之后，narrow操作之后就是本层卷积的结束，将得出的特征图作为下一层卷积的输入进行计算，重复之前操作%
    
    
       %综合前面提出的exchange以及narrow操作的优势，我们专门为轻量化网络设计了一种SINet Unit。
    %这种Unit可以无缝的嵌入到任何cnn网络构架中，做到在不减少网络精度的前提下大幅降低网络计算量。
    %%%%%%%%%%%%%%%%%%%%%
    %Unit内部不同组的信息交互关系如图2所示，其中绿色模块是unit内部的特征计算层，红色线条表示了我们独特的shortcut形式，展现了在没有引入任何额外计算量的情况下我们式如何实现了组间的信息交互。
    %Unit内部结构的深度方向信息交互设计如图3所示，其中红色H表示特征计算（conv+relu+bn），浅紫红色模块表示经过每一层特征计算层的输出特征处理模块，不同颜色特征表示不同层产生的特征,不同颜色的线条表示相应特征的信息流，可以看出随着层级的加深，后面每一层都会包含前面所有层的信息。
    %蓝色部分表示的是narrow操作（具体实现见图2中蓝色模块），这个操作紧连在每个层级的连接计算之后，为了可以在有限的计算资源下实现全联通的信息交互形式（图3显示了我们是如何实现每个unit单个组内部式如何实现全联通的）。
    %unit的整体结构如图5所示，我们结合使用了图2的组间信息交互以及图3的深度方向上层级之间的信息交。这种unit结构是一种具有dense funnel连接的倒置组间交互残差的瓶颈深度可分离卷积。
    %%%%%%%%%%%%%%%%%%%%%
    
    
    %经典的cnn网络可以分为三个部分：
%一系列级联的conv+pooling层。在级联的过程中，输入尺寸会逐渐变小，同时输出的channel数逐渐变大，完成信息从低级到高级的抽象。 一系列级联的全连接层。在卷积层到全连接层的交界处，卷积层输出会被转化成一维的输入送进全连接层。
% 最后的输出层，根据任务的需要，决定输出的形式。
%图1展示了传统的卷积神经网络在做分类任务的基本框架，可以看出经典cnn的全连接层使用的特征只是最后一层卷积层得到的特征，这是最高级的一种特征。
%对于卷积神经网络而言，用于决策的可利用特征应该要越全面越好，虽说高级特征可以较高程度的表征图片信息，但是这并不表示低级信息是没有用的，相反，这些低级信息应该被利用起来。
%也就是说将低级特征和高级特征进行有效的联合决策会提高深度网络的决策效果。
%一种最为直观的联合决策的方式就是不同层级的特征直接连接，这种简单的操作只能用在每一层特征图的大小不变时。然而，卷积网络的一个重要部分是下采样层，这些层改变了特征映射的大小。
% 为了将不同大小的特征图进行连接，一种简单的思想就是对于这些特征图进行不同程度的下采样，然后将下采样到统一尺度的特征度进行连接，最后用于决策。
%但是这种方法有一个缺点：首先，下采样得到的特征图已经失去了这一层级特征图特有的特征信息，再者，直接的下采样都会有一定程度的信息丢失，用失去了有效特征信息并且还有部分信息丢失的特征来结合最后的卷积特征进行决策，这会在一定程度上干扰网络的决策(添加引用实验表）。
%为了让各个层级的特征信息无损失的进行联合，我们将不同层级（Block）输出的特征图分别转化为一维的输出，然后将全部的一维特征直接连接起来输入全连接层。
%不同层级的特征信息的贡献对于网络最后的决策是不一样的，为了体现不同层级特征的贡献度，我们通过学习到不同层级特征的依赖关系来平衡其贡献度。
%
%贡献函数的目标是根据不同block的输入特征信息估计其特征的相关性。
%我们建立在最近的研究()上，这些研究表明卷积特征中的大部分信息是通过不同信道的统计及其相互依赖性来捕获的。
%我们只考虑通过全局平均汇集收集的渠道方式，即只考虑特征压缩为1×1×C通道描述符，所以直接在特征连接层进行贡献度的计算。
%为了捕获通道之间的依赖关系，我们添加了一个简单的非线性函数，它由两个完全连接的层连接，并与ReLU激活函数相连。此操作的输出是图层的贡献度分数。具体的。。。
%得到不同block输出特征的贡献度的分数后，将原本特征按照贡献度分数加权相加就是我们的基于atention的多尺度决策模块。


%基于SI unit和基于注意的分层联合决策中，我们在表中呈现整体SINet整体结构。
%Si unit采用的是分组计算，其基本构建块是具有反向残差的瓶颈深度可分离卷，我们的残差结构是一种新型的具有组间的信息交互的exchange shortcut连接；其基本构建快的连接形式我们采用的是一种新颖密集的漏斗层。
%我们提出的网络主要由分成四个阶段的一组SI单元组成。每个阶段的第一个构建块使用stride=2，与mobilenet2类似，我们使用扩展因子6应用于每个单元的输入张量大小。


	
%     And the specific implementation is introduced in Section \ref{Exchange Shortcut Connection}.
%     , and the specific implementation is introduced in Section \ref{dense funnel layer}
    
%     In SI Unit, the information interaction along depth direction is shown in Figure \ref{fig:narrow}. 
%     The light amaranth module presents the feature obtained from each block processing module through,
%     where the different color features represent the different layers, and the lines of different colors represent the information flow of different features. 
%     It can be seen that as the level deepens, each subsequent layer will contain information about all the previous units.
%     The blue part indicates the narrow operation which is closely connected to the connection calculation of each level, in order to realize the information exchange form of the full communication under the limited computing resources. 

% We also can downsample these feature maps into a fixed sizeto fuse them.
% However, this method also has a disadvantage: the feature maps obtained by downsampling has lost information which is unique to their level. It would lead to disturbance with the network classification \xu{add a reference to the experimental table}.

% This compresses the input features into 1 $\times 1 \times C$ channel (consider input feature maps is $H \times W \times C$)descriptor.


% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[h]
\centering
\caption{Bottleneck residual block transforming from k
to k' channels, with stride s, and expansion factor t.}
\begin{tabular}{rrr}
&         &  \\
\midrule
\multicolumn{1}{c|}{Input } & \multicolumn{1}{c|}{Operator } & \multicolumn{1}{c}{Output} \\
\midrule
\multicolumn{1}{c|}{h \times w \times k } & \multicolumn{1}{c|}{1 \times 1 conv2d , ReLU6 } & \multicolumn{1}{c}{h \times w \times (tk)} \\
\multicolumn{1}{c|}{\textit{h \times w \times tk }} & \multicolumn{1}{c|}{3 \times 3 dwise s=s, ReLU6 } & \multicolumn{1}{c}{\dfrac{h}{s} \times \dfrac{w}{s} × (tk)} \\
\multicolumn{1}{c|}{\dfrac{h}{s} \times w/s \times (tk)} & \multicolumn{1}{c|}{linear 1 \times 1 conv2d } & \multicolumn{1}{c}{\dfrac{h}{s} \times \frac{w}{s} \times k'} \\
\midrule
&         &  \\
\end{tabular}%
\label{tabel:Bottleneck residual block}
\end{table}%

%为了更好地验证各个单元的多功能性和有效性，我们还将其应用于4种不同的模型（包括2种轻量模型和2种传统模型），并分别比较它们的分类性能。
%值得注意的是，我们所有的参数量以及复杂度统计都是在标准的imagenet协议下测的（输入图片尺寸为224x224）。


%si unit主要贡献就是组卷积之后的exchange操作，以及exchange shortcut的dense funnel操作，为了验证si unit的有效性，我们将会如下设计实验。
%首先,
%在我们的实验中，我们将会对比原始网络，进行了分组操作的网络，利用了SI unit的网络。
%如表中所示，原始网络就是指组数设置为1的情况，当组数设置成2时，就表示进行了分组的操作。当EX设置为Y/N时，表示进行/不进行Exchange操作。
%从表中的结果可以看出，单纯的进行分组操作可以大幅降低网络的参数量以及计算量，但是同时会较多的损失原始网络的精度，而使用我们提出的exchange shortcut加上dense funnel结构的SI unit可以在网络参数量以及计算量的前提下，不损失甚至提高网络精度，这种表现在小型为网络中表现的更加好。
    

